Parameterized algorithms for identifying gene co-expression modules via weighted clique decomposition

We present a new combinatorial model for identifying regulatory modules in gene co-expression data using a decomposition into weighted cliques. To capture complex interaction effects, we generalize the previously-studied weighted edge clique partition problem. As a first step, we restrict ourselves to the noise-free setting, and show that the problem is fixed parameter tractable when parameterized by the number of modules (cliques). We present two new algorithms for finding these decompositions, using linear programming and integer partitioning to determine the clique weights. Further, we implement these algorithms in Python and test them on a biologically-inspired synthetic corpus generated using real-world data from transcription factors and a latent variable analysis of co-expression in varying cell types.

==> references.tex <==
% format: {first-author last name}{year}
% tie breaking:  {first-author last name}{year}{conf/journal abbr}


\begin{thebibliography}{99}

% NOTE: this format needs double checking!!
\bibitem{feldmann2020}
A.~E. Feldmann and D. Isaac and A. Rai {\em Fixed-Parameter Tractability of the Weighted Edge Clique Partition Problem}, 15th International Symposium on Parameterized and Exact Computation (IPEC 2020). Schloss Dagstuhl-Leibniz-Zentrum f{\"u}r Informatik, 2020.
\bibitem{offdiagonal}
Moutier, F., Vandaele, A. and Gillis, N., 2021. Off-diagonal symmetric nonnegative matrix factorization. Numerical Algorithms, pp.1-25.
\bibitem{zhang2013symmetricBMF}
Zhang, Z.Y., Wang, Y. and Ahn, Y.Y., 2013. Overlapping community detection in complex networks using symmetric binary matrix factorization. Physical Review E, 87(6), p.062803.
\bibitem{chen2021Instahide}
Chen, S., Song, Z., Tao, R. and Zhang, R., 2021. Symmetric Boolean Factor Analysis with Applications to InstaHide. arXiv preprint arXiv:2102.01570.
\bibitem{Kumar2019}
Kumar, R., Panigrahy, R., Rahimi, A. and Woodruff, D., 2019, May. Faster algorithms for binary matrix factorization. In International Conference on Machine Learning (pp. 3551-3559). PMLR.
\bibitem{Fomin2019ApxSchemes}
Fomin, F.V., Golovach, P.A., Lokshtanov, D., Panolan, F. and Saurabh, S., 2019. Approximation schemes for low-rank binary matrix approximation problems. ACM Transactions on Algorithms (TALG), 16(1), pp.1-39.
\bibitem{Ban2019Ptas}
	Ban, F., Bhattiprolu, V., Bringmann, K., Kolev, P., Lee, E. and Woodruff, D.P., 2019. {A PTAS for $\ell_p$-low rank approximation}. In Proceedings of the Thirtieth Annual ACM-SIAM Symposium on Discrete Algorithms (pp. 747-766). Society for Industrial and Applied Mathematics.
\bibitem{Fomin2020Parameterized}
Fomin, F.V., Golovach, P.A. and Panolan, F., 2020. Parameterized low-rank binary matrix approximation. Data Mining and Knowledge Discovery, 34(2), pp.478-532.
\bibitem{Miettinen2020Recent}
Miettinen, P. and Neumann, S., 2020. Recent developments in boolean matrix factorization. arXiv preprint arXiv:2012.03127.
\bibitem{Chandran2016Biclique}
Chandran, S., Issac, D. and Karrenbauer, A., 2017. On the parameterized complexity of biclique cover and partition. In 11th International Symposium on Parameterized and Exact Computation (IPEC 2016). Schloss Dagstuhl-Leibniz-Zentrum fuer Informatik.
\bibitem{fleischer2010K4Planar}
Fleischer, R. and Wu, X., 2010, November. Edge Clique Partition of K 4-Free and Planar Graphs. In International Conference on Computational Geometry, Graphs and Applications (pp. 84-95). Springer, Berlin, Heidelberg.
\bibitem{MujuniRosamond2008Kernel}
Mujuni, E. and Rosamond, F., 2008, January. Parameterized complexity of the clique partition problem. In Proceedings of the fourteenth symposium on Computing: the Australasian theory-Volume 77 (pp. 75-78).
\bibitem{Cygan2016ECC}
Cygan, M., Pilipczuk, M. and Pilipczuk, M., 2016. Known algorithms for edge clique cover are probably optimal. SIAM Journal on Computing, 45(1), pp.67-83.
\end{thebibliography}


==> sections/fig-guessk.tex <==
%Figure showing effect of incorrectly guessing k
\begin{figure}
\includegraphics[width=\linewidth]{figures/kguess-time_avg.pdf}
\caption{Effect of incorrectly guessing the input parameter $k$. Runtime ratio of incorrect guess over runtime on true $k$. The right of the plot shows overestimating the parameter, while the left shows understimating. 
The values at the middle point denote *Currently only showing LP on LV data*}
\label{fig:guessk}
\end{figure}

